High-resolution HST/ACS images of detached shells around carbon stars

Aims: The detached shells carry information on their formation process, as well as on the small-scale structure of the circumstellar medium around AGB stars due to the absence of significant line-of-sight confusion. Methods: The youngest detached shells, those around the carbon stars R Scl and U Cam, are studied here in great detail in scattered stellar light with the Advanced Survey Camera on the Hubble Space Telescope. Quantitative results are derived assuming optically thin dust scattering. Results: The detached dust shells around R Scl and U Cam are found to be consistent with an overall spherical symmetry. They have radii of 19.2" (corresponding to a linear size of 8x10^16 cm) and 7.7" (5x10^16 cm), widths of 1.2" (5x10^15 cm) and 0.6" (4x10^15 cm), and dust masses of 3x10^-6 and 3x10^-7 M(Sun), respectively. The dynamical ages of the R Scl and U Cam shells are estimated to be 1700 and 700 yr, respectively, and the shell widths correspond to time scales of 100 and 50 yr, respectively. Small-scale structure in the form of less than arcsec-sized clumps is clearly seen in the images of the R Scl shell. Average clump dust masses are estimated to be about 2x10^-9 M(Sun). Comparisons with CO line interferometer data show that the dust and gas shells coincide spatially, within the errors (<=1" for U Cam and approx. 2" for R Scl). Conclusions: The results are consistent with the interpretation of geometrically thin gas and dust shells formed by a mass-loss eruption during a He-shell flash, and where interaction with a previous wind plays a role as well. Clumpy structure is present in the R Scl shell, possibly as a consequence of the mass loss itself, but more likely as a consequence of instabilities in the expanding shell.

==> aasjournals.tex <==
%
%  These Macros are taken from the AAS TeX macro package version 4.0.
%  Include this file in your LaTeX source only if you are not using
%  the AAS TeX macro package and need to resolve the macro definitions
%  in the BibTeX entries returned by the ADS abstract service.
%
%  For more information on the AASTeX macro package, please see the URL
%       http://www.ferberts.com/AAS/aastex.html
%  For more information about ADS abstract server, please see the URL
%       http://adswww.harvard.edu/ads_abstracts.html
%

% Abbreviations for journals.  The object here is to provide authors
% with convenient shorthands for the most "popular" (often-cited)
% journals; the author can use these markup tags without being concerned
% about the exact form of the journal abbreviation, or its formatting.
% It is up to the keeper of the macros to make sure the macros expand
% to the proper text.  If macro package writers agree to all use the
% same TeX command name, authors only have to remember one thing, and
% the style file will take care of editorial preferences.  This also
% applies when a single journal decides to revamp its abbreviating
% scheme, as happened with the ApJ (Abt 1991).

\def\aj{\rm {AJ}}                   % Astronomical Journal
\def\araa{\rm {ARA\&A}}             % Annual Review of Astron and Astrophys
\def\apj{\rm {ApJ}}                 % Astrophysical Journal
\def\apjl{\rm {ApJ}}                % Astrophysical Journal, Letters
\def\apjs{\rm {ApJS}}               % Astrophysical Journal, Supplement
\def\ao{\rm {Appl.~Opt.}}           % Applied Optics
\def\apss{\rm {Ap\&SS}}             % Astrophysics and Space Science
\def\aap{\rm {A\&A}}                % Astronomy and Astrophysics
\def\aapr{\rm {A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\def\aaps{\rm {A\&AS}}              % Astronomy and Astrophysics, Supplement
\def\azh{\rm {AZh}}                 % Astronomicheskii Zhurnal
\def\baas{\rm {BAAS}}               % Bulletin of the AAS
\def\jrasc{\rm {JRASC}}             % Journal of the RAS of Canada
\def\memras{\rm {MmRAS}}            % Memoirs of the RAS
\def\mnras{\rm {MNRAS}}             % Monthly Notices of the RAS
\def\pra{\rm {Phys.~Rev.~A}}        % Physical Review A: General Physics
\def\prb{\rm {Phys.~Rev.~B}}        % Physical Review B: Solid State
\def\prc{\rm {Phys.~Rev.~C}}        % Physical Review C
\def\prd{\rm {Phys.~Rev.~D}}        % Physical Review D
\def\pre{\rm {Phys.~Rev.~E}}        % Physical Review E
\def\prl{\rm {Phys.~Rev.~Lett.}}    % Physical Review Letters
\def\pasp{\rm {PASP}}               % Publications of the ASP
\def\pasj{\rm {PASJ}}               % Publications of the ASJ
\def\qjras{\rm {QJRAS}}             % Quarterly Journal of the RAS
\def\skytel{\rm {S\&T}}             % Sky and Telescope
\def\solphys{\rm {Sol.~Phys.}}      % Solar Physics
\def\sovast{\rm {Soviet~Ast.}}      % Soviet Astronomy
\def\ssr{\rm {Space~Sci.~Rev.}}     % Space Science Reviews
\def\zap{\rm {ZAp}}                 % Zeitschrift fuer Astrophysik
\def\nat{\rm {Nature}}              % Nature
\def\iaucirc{\rm {IAU~Circ.}}       % IAU Cirulars
\def\aplett{\rm {Astrophys.~Lett.}} % Astrophysics Letters
\def\apspr{\rm {Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\def\bain{\rm {Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\def\fcp{\rm {Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\def\gca{\rm {Geochim. Cosmochim. Acta}}   % Geochimica Cosmochimica Acta
\def\grl{\rm {Geophys.~Res.~Lett.}} % Geophysics Research Letters
\def\jcp{\rm {J.~Chem.~Phys.}}      % Journal of Chemical Physics
\def\jgr{\rm {J.~Geophys.~Res.}}    % Journal of Geophysics Research
\def\jqsrt{\rm {J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{\rm {Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\def\nphysa{\rm {Nucl.~Phys.~A}}   % Nuclear Physics A
\def\physrep{\rm {Phys.~Rep.}}   % Physics Reports
\def\physscr{\rm {Phys.~Scr}}   % Physica Scripta
\def\planss{\rm {Planet.~Space~Sci.}}   % Planetary Space Science
\def\procspie{\rm {Proc.~SPIE}}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao


